DeGAS: Gradient-Based Optimization of Probabilistic Programs without Sampling

We present DeGAS, a differentiable Gaussian approximate semantics for loopless probabilistic programs that enables sample-free, gradient-based optimization in models with both continuous and discrete components. DeGAS evaluates programs under a Gaussian-mixture semantics and replaces measure-zero predicates and discrete branches with a vanishing smoothing, yielding closed-form expressions for posterior and path probabilities. We prove differentiability of these quantities with respect to program parameters, enabling end-to-end optimization via standard automatic differentiation, without Monte Carlo estimators. On thirteen benchmark programs, DeGAS achieves accuracy and runtime competitive with variational inference and MCMC. Importantly, it reliably tackles optimization problems where sampling-based baselines fail to converge due to conditioning involving continuous variables.

==> text/cfg.tex <==
\begin{figure}[htbp]
    \centering
    \begin{tikzpicture}[node distance=1.8cm, scale=0.8, every node/.style={transform shape}]
        % Styles
        \tikzset{
            circnode/.style={
                draw, circle, minimum width=1cm, minimum height=1cm, inner sep=0pt, 
                text width=1cm, align=center, font=\small
            },
            arrow/.style={-{Latex}}
        }

        % Nodes (arranged horizontally)
        \node[circnode] (entry) {$\node_0$ \\ $\entrytype$};

        \node[circnode, right=1.2cm of entry, label=below:{\shortstack{$x \sim gm([1], [0], [\sigma])$}}] 
            (rnd) {$\node_1$ \\ $\rndstatetype$};

        \node[circnode, right=1.2cm of rnd, label=below:{$x < \theta$}] 
            (test) {$\node_2$ \\ $\testtype$};

        \node[circnode, below right=0.5cm and 1.5cm of test, 
              label=below:{\shortstack{$y=-1$ \\ $\condfunc(\node)=\textit{false}$}}] 
              (det2) {$\node_4$ \\ $\detstatetype$};

        \node[circnode, above right=0.5cm and 1.5cm of test, 
              label=below:{\shortstack{$y=1$ \\ $\condfunc(\node)=\textit{true}$}}] 
              (det1) {$\node_3$ \\ $\detstatetype$};

        \node[circnode, right=3cm of test] 
              (exit) {$\node_5$ \\ $\exittype$};

        % Edges
        \draw[arrow] (entry) -- (rnd);
        \draw[arrow] (rnd) -- (test);
        \draw[arrow] (test) -- (det1);
        \draw[arrow] (test) -- (det2);
        \draw[arrow] (det1.east) -- (exit.north);
        \draw[arrow] (det2.east) -- (exit.south);
    \end{tikzpicture}
    \caption{Cfg of program $P$.}
    \label{fig:cfg}
\end{figure}


==> text/tabelle_50000_iters.tex <==
\begin{table}[H]
\centering
\begin{tabular}{l|cc|cccc|cc}
\toprule
\textbf{Model} &
\multicolumn{2}{c|}{\textbf{VI}} & 
\multicolumn{4}{c|}{\textbf{MCMC}} & 
\multicolumn{2}{c}{\textbf{DeGAS}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-7} \cmidrule(lr){8-9}
 & \textbf{LR} & \textbf{Steps}
  & \textbf{Samples} & \textbf{Warmup} & \textbf{R-hat} & \textbf{N eff} 
 & \textbf{LR} & \textbf{Steps} \\
\midrule
%\rowcolor{gray!20}
Bernoulli & $0.05$ & $247$ & $500$ & $50$ & $1.005$  & $802$ & $0.01$ & $248$ \\
Burglary  & $0.05$ & $50000$ & $500$ & $50$ & $1.003$ & $1008$  & $0.005$ & $295$ \\
%\rowcolor{gray!20}
ClickGraph & $0.001$ & $50000$ & $500$ & $50$ & $1.018$ & $333$ & $0.2$ & $216$\\
%\rowcolor{gray!20}
ClinicalTrial  & $0.2$ & $20013$ & $500$ & $50$ & $1.021$ & $146$ &  $0.001$ & $500$\\
Grass  & $0.0005$ & $50000$ & $500$ & $50$ & $1.004$  & $1444$ &  $0.1$ & $500$\\
%\rowcolor{gray!20}
MurderMistery  & $0.05$ & $26357$ & $500$ & $50$  & $1.001$ & $1036$ & $0.01$ & $239$\\
%\rowcolor{gray!20}
SurveyUnbiased  & $0.0005$ & $7211$ & $500$ & $50$ & $1.001$ & $1382$ & $0.01$ & $500$\\
%\rowcolor{gray!20}
TrueSkills  & $0.1$ & $50000$ & t.o. & t.o. & t.o. & t.o. & $0.2$ & $367$\\
%\rowcolor{gray!20}
TwoCoins  & $0.001$ & $50000$ & $500$ & $50$ & $1.015$ & $279$  & $0.001$ & $337$\\
%\rowcolor{gray!20}
AlterMu & $0.2$ & $50000$ & t.o. & t.o.  & t.o. & t.o.  & $0.05$ & $235$\\
%\rowcolor{gray!20}
AlterMu2  & $0.1$ & $50000$ & $1500$ & $50$  & $1.040$ & $81$ & $0.2$ & $228$\\
NormalMixtures & $0.0005$ & $50000$ & $500$ & $50$ & $1.018$& $457$ & $0.01$ & $500$\\
PID & $0.005$ & $50000$ & n.c. & n.c. & n.c. & n.c. & $0.2$ & $1000$ \\

\bottomrule
\end{tabular}
\caption{Tuned hyperparameters (see Section \ref{sec:experiments}) used for the synthesis of probabilistic program parameters.}
\label{tab:hyper}
\end{table}



\begin{table}[t]
\centering
\begin{tabular}{l|c|c|cc|cc|cc}
\toprule
\textbf{Model} & \textbf{\# Par.} & \textbf{\# Var.} &
\multicolumn{2}{c|}{\textbf{VI}} & 
\multicolumn{2}{c|}{\textbf{MCMC}} & 
\multicolumn{2}{c}{\textbf{DeGAS}} \\
\cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
 & & & \textbf{Time} & \textbf{Error}
 & \textbf{Time} & \textbf{Error} 
 & \textbf{Time} & \textbf{Error} \\
\midrule
\rowcolor{gray!20}
Bernoulli & $1$ & $2$ & $0.204$ & $0.024$ & $10.968$  & $0.023$& $1.986$ & $0.001$ \\
Burglary & $2$ & $7$  & $75.809$ & $0.913$ & $13.014$ & $0.141$  & $14.347$ & $1.686$ \\
\rowcolor{gray!20}
ClickGraph & $1$ & $6$ & $37.570$ & $0.376$ & $62.546$ & $0.096$ & $21.600$ & $0.086$\\
\rowcolor{gray!20}
ClinicalTrial  & $3$ & $6$ & $25.055$ & $1.954$ & $120.492$ & $2.536$ &  $17.070$ & $0.657$\\
Grass  & $4$ & $6$ & $83.595$ & $0.313$ & $58.151$ & $0.015$  & $317.582$ & $0.036$\\
\rowcolor{gray!20}
MurderMistery  & $1$ & $1$ & $11.807$ & $6.600$ & $14.036$ & $2.303$  & $2.508$ & $0.203$\\
\rowcolor{gray!20}
SurveyUnbiased  & $2$ & $2$ & $4.823$ & $0.009$ & $17.030$ & $0.013$  & $11.570$ & $0.008$\\
\rowcolor{gray!20}
TrueSkills & $3$ & $6$ & $64.132$ & $0.006$ & t.o. & t.o. & $1.664$ & $0.003$\\
\rowcolor{gray!20}
TwoCoins & $2$ & $1$ & $45.510$ & $0.981$ & $49.120$ & $0.873$  & $3.410$ & $0.688$\\
\rowcolor{gray!20}
AlterMu & $3$ & $5$ & $56.60$ & $1.672$ & t.o. & t.o. & $0.640$ & $0.312$\\
\rowcolor{gray!20}
AlterMu2 & $2$ & $3$ & $34.212$ & $1.488$ & $384.730$ & $0.139$  & $0.618$ & $0.096$\\
NormalMixtures & $3$ & $3$ & $51.916$ & $2.804$ & $345.409$ & $0.053$ & $2.941$ & $0.386$\\
PID & $2$ & $55$ & $3019.65$ & -- & nc & nc & $419.290$ & -- \\
\bottomrule
%\textbf{Avg.} & & 
\end{tabular}
\caption{Comparison of inference methods across models.
Models highlighted in gray indicate cases where DeGAS outperformed both other methods in either accuracy or execution time. For the last model, PID, we are not able to quantify the error, as the true parameters are unknown, but  we show the result of the optimization in Figure \ref{fig:PID_opt_reach}. MCMC fails to converge for this case study ($\hat{R} \gg 1$.)}
\label{tab:vi_mcmc_degas}
\end{table}
